Assessing the Helpfulness of Learning Materials with Inference-Based Learner-Like Agent

Many English-as-a-second language learners have trouble using near-synonym words (e.g., small vs.little; briefly vs.shortly) correctly, and often look for example sentences to learn how two nearly synonymous terms differ. Prior work uses hand-crafted scores to recommend sentences but has difficulty in adopting such scores to all the near-synonyms as near-synonyms differ in various ways. We notice that the helpfulness of the learning material would reflect on the learners' performance. Thus, we propose the inference-based learner-like agent to mimic learner behavior and identify good learning materials by examining the agent's performance. To enable the agent to behave like a learner, we leverage entailment modeling's capability of inferring answers from the provided materials. Experimental results show that the proposed agent is equipped with good learner-like behavior to achieve the best performance in both fill-in-the-blank (FITB) and good example sentence selection tasks. We further conduct a classroom user study with college ESL learners. The results of the user study show that the proposed agent can find out example sentences that help students learn more easily and efficiently. Compared to other models, the proposed agent improves the score of more than 17% of students after learning.

==> approach-orig.tex <==

\begin{table*}[]
\center \scalebox{0.53}{
\begin{tabular}{|c|m{10cm}|m{10cm}|p{1cm}|}
\hline
\textbf{Learner-Like Agent Type} & \multicolumn{1}{c|}{\textbf{Example Sentence}}& \multicolumn{1}{c|}{\textbf{Question}} &\multicolumn{1}{c|}{\textbf{Label}}                   \\ \hline\hline
\textbf{Entailment Modeling}                                 & After founding the Institute he had \textbf{[little]} time for composing, and appears to have concentrated exclusively on teaching.                                                                    & When she finds out the truth, she makes a fateful decision to make the most of the \textbf{[little]} time they have together.                 & \multicolumn{1}{c|}{\{$\mathbf{entail} \neg \mathit{entail}$\}} \\ \hline
\textbf{Context Modeling}                                    & After founding the Institute he had \textbf{[little]} time for composing, and appears to have concentrated exclusively on teaching. It makes me feel \textbf{[small]} when you keep things from me. & When she finds out the truth, she makes a fateful decision to make the most of the \textbf{\textsc{[MASK]}} time they have together. & \multicolumn{1}{c|}{\{$\mathbf{little}, small$\}}       \\ \hline
\textbf{Perturbing Example in Entailment}                    & After founding the Institute he had \textbf{[small]} time for composing, and appears to have concentrated exclusively on teaching.                                                                            & When she finds out the truth, she makes a fateful decision to make the most of the \textbf{[small]} time they have together.                         & \multicolumn{1}{c|}{
\{$\mathbf{entail},\neg \mathit{entail}$\}}  \\ \hline
\textbf{Perturbing Example in Context}                       & It makes me feel \textbf{[little]} when you keep things from me. After founding the Institute he had \textbf{[small]} time for composing, and appears to have concentrated exclusively on teaching.                & When she finds out the truth, she makes a fateful decision to make the most of the \textbf{\textsc{[MASK]}} time they have together. & \multicolumn{1}{c|}{\{$little, \mathbf{small}$\}}       \\ \hline
\textbf{Bad Example} & \multicolumn{1}{c|}{\textbf{Example Sentence}}& \multicolumn{1}{c|}{\textbf{Question}} &\multicolumn{1}{c|}{\textbf{Label}}                   \\ \hline\hline                    
\multicolumn{1}{|c|}{\textbf{Entailment Modeling}} & After founding the Institute he had \textbf{[small]} time for composing, and appears to have concentrated exclusively on teaching.                                                                            & When she finds out the truth, she makes a fateful decision to make the most of the \textbf{[little]} time they have together.                         & \multicolumn{1}{c|}{$\{entail, \mathbf{\neg entail}$\}} \\ \hline
\textbf{Context Modeling}                          & It makes me feel \textbf{[little]} when you keep things from me. After founding the Institute he had \textbf{[small]} time for composing, and appears to have concentrated exclusively on teaching.                & When she finds out the truth, she makes a fateful decision to make the most of the \textbf{\textsc{[MASK]}} time they have together. & \multicolumn{1}{c|}{\{$\mathbf{little}, small$\}}       \\ \hline
\end{tabular}}
\caption{The example of training instances for different learner-like agents
are provided.}
%This table illustrates all text examples we used in the paper in the following order: natural language inference, learner-like agent by types (Section \ref{sec:ENT}), generated bad example (Section \ref{subsec:behave-check}), and fill-in-the-blank for user study (Section \ref{sec:learner}) example.}

%The inputs of different question design for the learner-like agents are demonstrated in row 1-4. (\textsc{[cls]} is inserted in the beginning of example sentence, and \textsc{[sep]} wraps the question sentence.) In this example, we only show one pair of examples instead of three for \fitb{} and one example instead of six for \ent{}. We also show other example cases and fill-in-the-blank question templates, which we will discuss in the paper. 

\label{tab:agent_example}
\end{table*}

In this paper, we call a model with the ability to answer questions based on
given examples, a learner-like agent. We propose to use \ent{} on the
learner-like agent because human behavior originated from the capability of
inference, and \ent{} utilizes the inference concept. We will describe the
pre-trained model we build upon, define our learner-like agent and \ent{}, and
introduce the perturbing instances used to enhance the agent's
learner-behavior.

Pre-trained language models have shown to be effective for learning universal
language representation. A pre-trained bidirectional transformers BERT
model~\cite{devlin2018bert} can be find-tuned to create state-of-the-art models
for a range of natural language understanding tasks, such as question answering
and natural language inference.  Thus, we adopt Devlin's BERT
model(\citeyear{devlin2018bert}) to fine-tune on our learner-like agent
task-specific layer using our training data. This fine-tuning will equip the
learner-like agent the ability to acquire the near-synonym difference.

\subsection{Learner-Like Agent}
\label{subsec:learner_like_agent}

The overall structure of a learner-like agent is as follows: given six example
sentences $\mathbb{E}$ (3 sentences for each word) and a question $Q$ as an
instance for input, the model should answer the question based on the example
hints. 


The input of our model contains:
\begin{itemize}
\item A question $Q^{w_i} = [q_1, q_2, .., q_n]$, where $n$ is the length of
the sentence and contains a word $w_i$ from the near-synonym pair, where $i \in
\{1,2\}$ denotes word 1 or word 2;
\vspace{-2mm} 
\item Example sentences set $\mathbb{E} =[E^{w_1}_{1}, ..., E^{w_1}_{3},
E^{w_2}_{4}, ..., E^{w_2}_{6}]$, where $E^{w_i}$ denotes a  sentence containing
$w_i$;  \vspace{-2mm}
\item A \textsc{[cls]} token for the classification position, and several
\textsc{[sep]} tokens used to label the boundary of the question and the
example sentences from BERT setting.
\end{itemize}

We specifically define $E[w_j]^i$ where $i, j \in {1,2}$. For example,
$E[w_1]^2$ is a example sentence where $w_1$ is filled in the position of $w_2$
in $E^{w_2}$ sentence. This notation also applies to the question input
$Q[w_j]^i$.



%replacing $w_i$ position to a blank.

%We also represent context of ${w_1}$ as $E[\_]^i$, context of ${w_2}$ as $E[\_]^2$, leaving original $w_i$ position a blank $[\_]$ to fill with either ${w_1}$ or ${w_2}$ . This notation also applies to the question input $Q[\_]^1$ and $Q[\_]^2$ .

%For instance, an input of Learner-Like Agent can be:

%\begin{quote}
%\small
%\textsc{[cls]} After founding the Institute he had [little] time for composing, and appears to have concentrated exclusively on teaching. \textsc{[sep]}
%When she finds out the truth, she makes a fateful decision to make the most of the [little] time they have together. \textsc{[sep]}
%\end{quote}
%In this example, we only show one example instead of six. The learner-like agent answers differently in different question design. In \ent{}, the question design asks the model to answer the relationship between question and example.

\subsection{Inference-based Entailment Modeling}
%In NLI task, it asks whether a premise entails a hypothesis. For example, given a premise, \say{A man inspects the uniform of a figure in some East Asian country.} and a hypothesis \say{The man is sleeping.}, a model should answer \textit{contradiction}. RQE, on the other hand, identifies entailment between two questions in the context of QA. \joy{Should I move the example to Table 1? already up there, but not sure if it fits}

We apply NLI and RQE tasks in the learner-like agent question design. The goal
of the \ent{} learner-like agent is to look at example sentences and answer the
entailment questions. 
An entailment question for \ent{} is a sentence, and the model predicts if
example sentence $E$ entails the question sentence $Q$. If the target word and
its context follows example suggestion, the \ent{} model answers
$\mathit{entail}$, or $\neg \mathit{entail}$ otherwise. 

The \ent{} model $M_e$ is described as:
\begin{equation}
    M_e(E^{w_i}_j, Q^{w_j}) = ans 
\end{equation}
where $ans$, either $entail$ or $\neg \mathit{entail}$, is the prediction of
the inference relationship of one of the six example sentence $E^{w_i}_i$ and
$Q^{w_j}$.
To fill all the context possibilities of $Q[\_]^i$ for the same word in
$E^{w_i}$, an example has four cases. The corresponding example cases are:
\begin{align}
    &M_e(E[w_1]^1,Q[w_1]^1) = \mathit{entail} \label{eqn:eq2} \\
    &M_e(E[w_1]^1,Q[w_2]^2) = \neg \mathit{entail} \label{eqn:eq3} \\
    &M_e(E[w_1]^1,Q[w_2]^1)) = \neg \mathit{entail} \label{eqn:eq4} \\
    &M_e(E[w_1]^1,Q[w_1]^2) = \neg \mathit{entail} \label{eqn:eq5}
\end{align}

From the input and output of instances (Equation \ref{eqn:eq2} to
\ref{eqn:eq5}), we can see that the target word and their context in $Q$ for
all cases except Equation \ref{eqn:eq2} do not follow example word suggestion.
%In equation \ref{eqn:eq3}, the context is not similar, and word usage is different, so the model cannot guarantee that it is correct; therefore, the relation is \textit{not entail}. In equation \ref{eqn:eq4}, the context is similar, but word usage is different, thus \textit{not entail}. In equation \ref{eqn:eq5}, the context is not similar, and word usage is incorrect given example word usage, therefore \textit{not entail}. We illustrate a example and its question with label of \ent{} in Table \ref{tab:agent_example}.


%Taking the example mentioned in \ref{subsec:learner_like_agent}, the near-synonym wordpair is \textit{little} and \textit{small}. The answer to such a pair is \textit{entail}. If the question sentence changes to \say{When she finds out the truth, she makes a fateful decision to make the most of the [small] time they have together.}, the model should answer \textit{not entail}. 

%Recall that the purpose of a learner-like agent is to infer the relationship between a question and example pair and apply it to learn the near-synonym difference.
Besides making \ent{} learner-like agent to understand the relation between
example and question, we can convert its prediction \{$\mathit{entail}$, $\neg
\mathit{entail}$\} back into the lexical choice by looking into the model
predictions.
Given the probability of \{$\mathit{entail}$, $\neg \mathit{entail}$\}, we can
know which term in the near-synonym pair is more appropriate in $\{Q[\_]^1,
Q[\_]^2\}$ context. If the question context and the example context matches,
then a word with a higher $\mathit{entail}$ probability will be the answer. If
not matches, the one with higher $\neg \mathit{entail}$ probability is the
answer. 

\subsection{Perturbing Instance}

\label{subsec:perturbing_example}
To encourage learner-like behavior, i.e., good examples lead to the correct
answer, and vice versa, we proposed to introduce automatic generated perturbing
instances in the training process.

If we carefully look at the input and output of instances (Equation
\ref{eqn:eq2} to \ref{eqn:eq5}), we can find they only consider good examples
and their corresponding labels. We postulate that wrong word usage makes bad
examples and create perturbing instances by the concept of swapping the current
confusing word to its  near-synonym as 
\begin{equation}\vspace{-2mm}
    M_e(E[\neg w_i]^{w_i}_j, Q^{w_j}) = \mathit{\neg ans}
\end{equation}
where $\mathit{\neg ans}$ is \{$entail,\neg entail$\}- $\mathit{ans}$, and
$E[\neg w_i]^{w_i}_j$ is the example sentence in which the context in 
$w_1$ and $w_2$ are swapped. 
%Thus when providing the perturbing example, a model should predict the opposite answer since that is what the perturbing example sentences demonstrate. The model should always assume example sentences are correct. 
As a result, the corresponding perturbing instances from Equation \ref{eqn:eq2}
to \ref{eqn:eq5} are 
\begin{align}
    &M_e(E[w_2]^1,Q[w_1]^1) = \neg \mathit{entail} \label{eqn:eq6}\\
    &M_e(E[w_2]^1,Q[w_2]^2) = \neg \mathit{entail} \label{eqn:eq7}\\
    &M_e(E[w_2]^1,Q[w_2]^1) = \mathit{entail} \label{eqn:eq8}\\
    &M_e(E[w_2]^1,Q[w_1]^2) = \neg \mathit{entail} \label{eqn:eq9}
\end{align}

, respectively, where which $w_2$'s context becomes $E[\_]^1$.

%In equation \ref{eqn:eq6}, the environment is similar, but the word usage is not guaranteed to be correct, therefore not entail. 
% In equation \ref{eqn:eq7}, the environment is not similar, but the word usage is not a properly given example, therefore \textit{not entail}. 
%In equation \ref{eqn:eq8}, the environment is similar, and the word usage correct; therefore, the example entails the question. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% comment
			\begin{comment}

			\begin{equation}\label{eqn:eq2}
			(E[w_1]_1,Q[w_1]_1) = \mbox{entail}\vspace{-2mm}
			\end{equation}
			\begin{equation}\label{eqn:eq3}
			(E[w_1]_1,Q[w_2]_2) = \mbox{not entail}\vspace{-2mm}
			\end{equation}
			\begin{equation}\label{eqn:eq4}
			(E[w_1]_1,Q[w_2]_1) =\mbox{not entail}\vspace{-2mm}
			\end{equation}
			\begin{equation}\label{eqn:eq5}
			(E[w_1]_1,Q[w_1]_2) =\mbox{not entail}
			\end{equation}


			\begin{equation}\label{eqn:eq6}(E[w_2]_1,Q[w_1]_1) = \mbox{not entail}
			\end{equation}\vspace{-2mm}
			\begin{equation}\label{eqn:eq7}(E[w_2]_1,Q[w_2]_2) = \mbox{not entail}
			\end{equation}\vspace{-2mm}
			\begin{equation}\label{eqn:eq8}(E[w_2]_1,Q[w_2]_1)) = \mbox{entail}
			\end{equation}\vspace{-2mm}
			\begin{equation}\label{eqn:eq9}(E[w_2]_1,Q[w_1]_2) = \mbox{not entail}
			\end{equation}

			\end{comment}


==> conclusion-orig.tex <==
We introduce the learner-like agent, especially \ent{}, which discerns the
helpfulness of learning materials using inference ability. 
Entailment modeling, unlike common context-based near-synonymous word
disambiguation, can make the inference to learn the relationship between
example sentence and question, similar to human behavior. Context modeling on
learner-like agent relies upon additional perturbing examples to mimic human
behavior while \ent{} already have the capability. The agent can be used to
evaluate the helpfulness of learning materials, or, more interestingly, to
select the best materials from a large candidate pool. We select good example
sentences in practice, which confirms the usefulness of modeling learner
behavior. Using the \ent{} learner-like agent, we find more helpful learning
material for learners, as demonstrated by the learner-study. These confirm the
usefulness of modeling learner behavior using the inference approach.


==> experiments-orig.tex <==
We conducted three experiments: ({\em i}) lexical choice, ({\em ii}) behavior
check, and ({\em iii}) sentence selection. 
The lexical choice task assesses whether the model can differentiate confusing
words.
Behavior check measures whether the model can respond to the qualities of
learning material like learners.
Sentence selection evaluates the model's ability to explore useful example
sentences.

% We evaluates whether a model can understand the difference between near-synonym wordpairs using lexical choice task. Thus, we used it as our standard task and trained the model on it. After the model acquires the near-synonym, we test whether the model can respond to the different quality of learning material in terms of behavior. Lastly, the sentence selection evaluated selected sentences to verify the usefulness of learner behavior modeling. 

\subsection{Lexical Choice}
The lexical choice aims at evaluating the model's capability of differentiating
confusing words.
The fill-in-the-blank task was used where the model needed to choose a word
from a given near-synonym wordpair to fill up the blank.

\subsubsection{Baseline}
\label{subsec:FITB}
\expandafter\MakeUppercase\fitb{} is a common practice for near-synonym
disambiguation in which the model learns the context of the target word through
the fill-in-the-blank task. 
Therefore developed a \textbf{Context Modeling} model as the baseline by using
BERT \cite{devlin2018bert} as a two-class classifier to predict that either
using $w_1$ or $w_2$ is more appropriate from a given word pair. 
% $w1$ or $w2$ is a word from given near-synonym word pair. 
The question for the context modeling model is a sentence whose target word,
i.e., one of the confusing words, is masked, and the model will predict the
masked target word. 

%Therefore, $Q[\textsc{MASK}]^{w_i}$ fills the the position of ${w_i}$ with \textsc{MASK}. 

The context modeling model $M_c$ is described as

\begin{equation}
    M_c(\mathbb{E}, Q[\textsc{mask}]^{i}) = \mathit{ans},
\end{equation}
where $Q[\textsc{mask}]^{w_i}$ fills the the position of ${w_i}$ with
\textsc{mask}, and ${ans} \in \{w_1,w_2\}$ is the prediction of the
\textsc{[mask]} in the question, and $\mathbb{E}$ are the 6 example sentences. 

%$\mathit{ans} \in \{w_1,w_2\}$ is the prediction of the \textsc{[mask]} in the
%question, $Q[\_]^{w_i}$ is the question whose  ${w_i}$ target word is masked, 
A $Q[mask]^{i}$ can be either a question with context of ${w_i}$ or ${w_2}$ .
This raise a problem. 
\begin{align}
\vspace{-3mm}
   & M_c(\mathbb{E}, Q[mask]^1) = w_1 \label{eq:cxt1}\\
   & M_c(\mathbb{E}, Q[mask]^2) = w_2
\label{eq:cxt2}
\vspace{-3mm}
\end{align}
%where $Q_1$ and $Q_2$ are questions that contain $w1$ and $w2$ respectively. 
Again, to encourage the learner-like behavior, we incorporate perturbing
instances in the training process corresponding to Equation~\ref{eq:cxt1}
and~\ref{eq:cxt2} as follows:
\vspace{-3mm}
\begin{align}
    &  M_c(\neg \mathbb{E}, Q[mask]^1) = w_2 \label{eq:ctx3}\\
    &  M_c(\neg \mathbb{E}, Q[mask]^2) = w_1  \label{en:ctx4}\vspace{-3mm}
\end{align},
where $\neg \mathbb{E}= [E[w_1]^2_1,...,E[w_1]^2_3,E[w_2]^1_1,...,E[w_2]^1_3]$.

% As shown above, the context modeling learner-like agent can predict the answer by only looking at the question. To explain in detail, if every input instance with question $Q_1$ has the answer $w_1$, the model will found out that it does not need to know the examples to answer correctly. 
For \fitb{}, the perturbing instance brings an additional benefit that it
forces the model making inference based on the given example sentences. Without
these instances, Equation~\ref{eq:cxt1} and~\ref{eq:cxt2} risk the model to
select $w_i$ given $Q_i$. 

%In addition to \ent{} learner-like agent and \fitb{} learner-like agent, we also trained one of each modeling without perturbing instances setting. The purpose is to see the effect of two models and the effect of perturbing instances. \joy{duplicate in dataset and setti up }

% \begin{equation}
%     \mathit{!ans} = M(!E, \textbf{Q)}
% \vspace{-3mm}
% \end{equation}
% on FITB input of the near-synonym set \textit{duty,task},
% $w1$ example sentence is \say{Determining the time at which two proteins diverged is an
% important [\textbf{duty}] in phylogenetics};
% $w2$ example sentence is \say{WSW was responsible for typical military
% counterintelligence and military police [\textbf{tasks}]};
% Question is \say{In cooperative mode, players alternate between both
% characters to solve puzzles and complete \textsc{[mask]}}.
% Here the agent should answer \textit{duty}. 

\subsubsection{Dataset and Settings}
We collected a set of near-synonym word pairs from online resources, including
BBC\footnote{\scriptsize
http://www.bbc.co.uk/learningenglish/chinese/features/q-and-a}, Oxford
Dictionary\footnote{\scriptsize
https://en.oxforddictionaries.com/usage/commonly-confused-words}, and a
Wikipedia page about commonly misused English words~\footnote{\scriptsize
shorturl.at/cmyG0}. 

Thirty near-synonym word pairs are manually selected as our experimental
material by an expert in ESL education.
We collected our data for both training and testing from Wikipedia on January
20, 2020. Words in the confusing word set usually are of the specific part of
speech. Therefore, we assure the part of speech of the confusing word in the
sentence pool matches that in target near-synonym word set. 
To construct a balanced dataset, we randomly selected 5,000 sentences for each
word; 4,000 sentences for each word in a near-synonym word pair are used for
training the learner-like model and 1,000 sentences for testing. 

We trained four learner-like agents, \ent{}, \fitb{}, \ent{} without perturbing
instances, and \fitb{} without perturbing instances, for comparison. We
empirically set the ratio of normal versus perturbing instances to $2:1$ for
the best learning effect.
Those learner-like agents are trained with the Adam optimizer with 30\% warm-up
proportion and 5e-5 learning rate. The maximum total input sequence length
after tokenization is 256, while other settings follow BERT's configuration. 

\subsubsection{Results and Discussion}
We compare \ent{} to the \fitb{} learner-like agents.
Figure \ref{fig:model_performance} shows the model performance on 30 word
pairs. The average accuracy of \ent{} and \fitb{} is 0.90 and 0.86, while that
excluding perturbing instances is 0.80 and 0.86, respectively. 
On average, \ent{} performs the best, and when perturbing instances are not
included in the training, its performance for lexical choice drops.  
We have expected that training with perturbing instances may reduce the models'
performance in exchange for learner-like behavior. 
However, results show that considering perturbing instances enhances \ent{}'s
ability to infer.
On the other hand, \fitb{} models seem to be not affected by perturbing
instances (yellow line vs. green line), and the possible reason could be that
\fitb{} tends to memorize the input context instead of making the inference,
which is also known as the bias in natural language inference
\cite{Chien_2020}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{figures/model_performance_by_wordpair.png}
	 \caption{Lexical choice performance visualization by all models from all
	 thirty near-synonym wordpairs are provided. }
    \label{fig:model_performance}
\end{figure}

\subsection{Behavior Check}
\label{subsec:behave-check}
\begin{table}[t]
\small \center
\addtolength{\tabcolsep}{-0.1cm}
\begin{tabular}{|c|c|c|}
\hline
                   & \textbf{T-score} & \textbf{P-value} \\ \hline
Context Modeling              & 24.54    & 2.06E-21 \\ \hline
Context Modeling w/o perturbing     & 0.77     & 0.45     \\ \hline
Entailment Modeling         & 92.12    & 2.43E-37 \\ \hline
Entailment Modeling w/o perturbing & 27.06    & 3.96E-22 \\ \hline
\end{tabular}
\addtolength{\tabcolsep}{0.1cm}
\caption{All models except \fitb{} w/o perturbing instances can response to the
change of learning material quality.}
\label{table:behavior_check_result}
\end{table}

The behavior check evaluates whether the agent learns like learners, that is, a
learner-like agent should perform well on the
fill-in-the-blank quiz when the given learning materials are helpful, and vice
versa.

In this experiment, all models are requested to do two fill-in-the-blank
quizzes.
For the first fill-in-the-blank quiz, authentic sentences are provided as good
learning materials; for the second quiz, bad learning materials are provided.
These materials for the second quiz are considered bad quality as they are
automatically generated using the same authentic sentences by replacing their
target words with near-synonyms for training, resulting in confusion and wrong
word usage as illustrated in Table \ref{tab:agent_example} (see "Bad Example in
Entailment" and "Bad Example in Context"). 
In other words, given bad example sentences, the model should select the other
choice of the same quiz question if it is capable of inferring answers from
these examples.

% \subsubsection{Artificial Counter Example}
% In this paper, the helpful learning materials refer to good example sentences. But what is good example? According to Kilgarriff et al. (\citeyear{kilgarriff2008gdex}), a good dictionary example must be :
% \begin{itemize}
% \item typical, exhibiting frequent and well-dispersed patterns of usage\vspace{-2mm}
% \item informative, helping to elucidate the definition\vspace{-2mm}
% \item intelligible to learners, avoiding gratuitously difficult lexis and structures, puzzling or distracting names, anaphoric references or other deictics which cannot be understood without access to the wider context. 
% \end{itemize}
% On top of those, there is a quality that is necessary especially for near-synonym: \textbf{``interchangeability''}. If a sentence's target word can be interchange by its near-synonym, it is not a good example. 
% \cy{\^ This doesn't looks related to this experiment?}

%The bad example can be automatically created by swapping the target word with its near-synonym, causing wrong word usage. 
%\lwku{combine the following to the union example?}\joy{modified}
%For instance, when the word set \textit{responsibility, liability} has a good example sentence:  
%\say{In the case of a limited \textbf{[liability]} company, an executive officer is any member, manager, or officer.},
%we can simply swap \textbf{liability} with \textbf{responsibility} to create a bad example sentence.
% Given the question 
% \say{The Panic of 1890 forced the bank to change from a partnership to an unlimited \textsc{[mask]} company in 1892}, 
% the agents should predict the gold answer \textit{liability}. 

\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{.45\linewidth}
    \includegraphics[width=1.0\columnwidth]{figures/ENT_behavior_check_0602_v2.png}
    \caption{Entailment Modeling}
    \end{subfigure}
    \begin{subfigure}[b]{.45\linewidth}
    \includegraphics[width=1.0\columnwidth]{figures/ENT_NC_behavior_check_0602_v2.png}
    \caption{Entailment Modeling w/o perturbing}
    \end{subfigure}
    \begin{subfigure}[b]{.45\linewidth}
    \includegraphics[width=1.0\columnwidth]{figures/FITB_behavior_check_0530_v2.png}
    \caption{Context Modeling}
    \end{subfigure}
    \begin{subfigure}[b]{.45\linewidth}
    \includegraphics[width=1.0\columnwidth]{figures/FITB_NC_behavior_check_0602_v2.png}
     \caption{Context Modeling w/o perturbing}
     \end{subfigure}

	 \caption{Behavior check visualization by results of model doing quiz when
	 good and bad learning materials are provided. Blue for learning with good
	 materials and orange for learning with bad materials. The x axis is the
	 quiz ID. Each quiz is conducted 11250 times (375 example sentence set for
	 each of 30 word sets).}
    \label{fig:behavior_check}
\vspace{-3mm}
\end{figure*}
\subsubsection{Results and Discussion}


% . We assume them to be good learning materials. 
% The other fill-in-the-blank quiz consists of the same sentence in good fill-in-the-blank quiz except all target word are replaced with its near-synonym term. 
% We evaluated the reactions of learning by these two fill-in-the-blank quizzes to baseline \fitb{} learner-like agents and \ent{} with and without perturbing instance setting.  

We record the accuracy of every question and combine 30 pairs of near-synonym
wordsets from the same model into one graph. As shown in Figure
\ref{fig:behavior_check}, we notice that even without perturbing instances, the
learning effect of \ent{} can correspond to the learning material quality. On
the other hand, \fitb{} without perturbing instances, like in the lexical
choice task, does not become worse when given bad examples.

To determine whether the accuracies of doing the two fill-in-the-blank quizzes
when providing good and bad examples are significantly different, We run a
t-test. Results shown in Table \ref{table:behavior_check_result} show that the
learner-like behavior is enabled in \fitb{} with perturbing instances, while
\ent{} learns like learners even without perturbing instances. This result
conforms to those are shown in Figure \ref{fig:behavior_check}. Results of two
quizzes for both \ent{} models can be clearly distinguished, while adding the
perturbing instances to \ent{} slightly enlarges their difference. Yet, the
\fitb{} still relies on perturbing instances to learn the difference. 

To look more closely, we present Table \ref{tab:behavior_result_by_wordpair}.
$\Delta$ is the accuracy difference of two quizzes. The higher $\Delta$ is, the
better the model knows the difference of confusing words. We measured the
correlation between the lexical choice accuracy and $\Delta$ with the Pearson
correlation coefficient and obtain its value 0.87, which demonstrates a strong
positive correlation.

\begin{table*}[]
\center
\scalebox{0.75}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
                              & \textbf{Acc} & \textbf{$\Delta$} &                         & \textbf{Acc} & \textbf{$\Delta$} &                            & \textbf{Acc} & \textbf{$\Delta$} \\ \hline
accountability, responsibility & 0.83   & 0.76  & traffic, transportation  & 0.89   & 0.80  & duty, task                  & 0.92   & 0.84  \\ \hline
particular, peculiar           & 0.84   & 0.73  & tiny, little             & 0.90   & 0.79  & real, authentic             & 0.92   & 0.86  \\ \hline
previous, former               & 0.86   & 0.76  & elder,elderly           & 0.90   & 0.80  & particular, specific        & 0.92   & 0.86  \\ \hline
elder, senior                  & 0.86   & 0.79  & creativity, innovation   & 0.90   & 0.83  & briefly, shortly            & 0.92   & 0.85  \\ \hline
small, little                  & 0.87   & 0.71  & common, ordinary         & 0.91   & 0.82  & decoration, ornament        & 0.93   & 0.87  \\ \hline
special, specific              & 0.88   & 0.74  & senior, elderly          & 0.91   & 0.82  & duty, job                   & 0.93   & 0.86  \\ \hline
accountability, liability      & 0.88   & 0.79  & acknowledge, admit       & 0.91   & 0.81  & achievement, accomplishment & 0.93   & 0.88  \\ \hline
specific, peculiar             & 0.89   & 0.73  & opportunity, possibility & 0.91   & 0.82  & responsibility, liability   & 0.94   & 0.88  \\ \hline
career, job                    & 0.89   & 0.80  & delay, postpone          & 0.91   & 0.82  & commitment, responsibility  & 0.94   & 0.88  \\ \hline
traffic, transport             & 0.89   & 0.80  & task, job                & 0.92   & 0.83  & cooperation, collaboration  & 0.95   & 0.89  \\ \hline
\end{tabular}}
\caption{Mapping of lexical performance and model's ability to differentiate
near-synonym for 30 word pairs using \ent{}}
\label{tab:behavior_result_by_wordpair}
\end{table*}


\subsection{Sentence Selection}
\label{subsec:sentence-selection}
In the sentence selection experiment, we evaluate the ability of the
learner-like agent in selecting useful example sentences. Our assumption is
straightforward. We give the developed learner-like agent a set of example
sentences and test its performance on a number of quizzes. If the agent can do
well in many quizzes, the example sentences are helpful for learning confusing
words. 

\subsubsection{Baseline}
We compare learner-like agents with an implementation of
Huang\shortcite{huang2017towards}'s \textbf{Gaussian mixture model}(GMM).
Huang's GMM learns the distribution and the semantic of the context. We set the
number of  Gaussian mixtures to 10 in GMM and trained the GMM with the dataset
in our paper. In the testing phase, we retrieved the top 3 recommend sentences
for each word in the confusing word set and compared it to the expert's
choices.

\subsubsection{Evaluation Dataset}
To evaluate the sentence selection, we employ two ESL teachers as experts to
carefully select three best example sentences out of ten randomly selected,
grammatically, and pragmatically correct examples for each word in all
confusing word pairs. 
%We request experts to select those that can clearly clarify the semantic difference between near-synonyms.
 
Specifically, the evaluation dataset has a total of 600 example sentences. For
each near-synonym pair, three sentences for each word are labeled as good
example sentences. To select sentences that can clearly clarify the semantic
difference between near-synonyms, the ESL expert considers
“\textit{suitability},” “\textit{informative},” “\textit{diversity},”
“\textit{sentence complexity},” and “\textit{lexical complexity}” during
selection. For \textit{suitability}, the expert considers whether the two
near-synonym words in one confusing word set are interchangeable in the current
sentence. The diversity is considered when constructing the selected pool.
Other criteria are from Kilgarriff's good example
sentence~\cite{kilgarriff2008gdex}. 
 
%[Turkers version] After consulting with two ESL education experts, we agree with an annotation guideline (see appendix) and uses for Amazon Mechanical Turkers. In a human intelligence task, we have three stages. In the first stage, we evaluate how well they understand the difference of the near-synonyms pair. In the second stage, we ask them to give each sentence a condition if the sentence fails to be a good sentence, otherwise the sentence should be acceptable. In the third stage, they selected the best three sentences out of the acceptable sentences. The agreement of this annotation is []. Such a dataset provides automatic evaluation for future research, and makes it possible if the model changes and when other researchers join the near-synonym example extraction task. 

\subsubsection{Selection Method}
We select a example sentence combination that can help \ent{} or \fitb{} models
to achieve the highest accuracy in the quiz as the proposed good example
sentence set. 

%Based on the learner-like agent structure design, an input instance has six example sentences and one question. To see which three sentences from the randomly selected examples for each word perform the best,  
One in a total of 14,400 ($C^{10}_3 \times C^{10}_3$) example sentence sets,
including 6 example sentences, are provided to the models for testing their
helpfulness. Each example sentence set will work with a quiz composed of $k$
questions. 
%The agent picks the combination that achieves the highest total testing. 
Here, the size of $k$ determines the representative and consistency of the
testing result from each quiz. 
%We are looking for a $k$ that covers more questions while keeping the example sentence combination’s response consistent. To do so, instead of performing on only one post-study quiz,
We use five independent quizzes to find a reliable $k$ by calculating the
correlation of their testing results. Finally, we empirically set $k$ to 100,
where the lowest correlation among 30 wordpairs is 0.24, and the median is
0.67. That is, there are 100 questions in each quiz.

When testing example sentence sets, there could be more than one set achieving
the highest accuracy for the quiz. All the sentences in these sets are proposed
as good example sentences and compared to gold labels for evaluation. 

%We calculate the correlation of the quiz score along with these five post-study quizzes. After comparing $k=\{10, 20, 30, ..., 100\}$, we choose $k=100$. When $k=100$, 

%Precision, recall, and F1 score are .

%\joy{Setting Two: Most Common}
%We collect all highest-score candidate-combinations and find the most common three sentences of each word to be the final selected example. And we compare the model's selection with expert choice in term of precision, recall, and F1 score.

\subsubsection{Result and Discussion}

Table~\ref{table:sentence_selection_result} shows the results of sentence
selection. 
%Both \ent{} and \fitb{} can mimic human behavior, as shown in the previous behavior check experiment. 
\expandafter\MakeUppercase\ent{} significantly outperforms \fitb{} and Haung's
GMM in sentence selection. The improvement comes from the increasing recall,
indicating the proposed learner-like agent manages to find helpful example
sentences for ESL learners. 
\begin{table}[h!]
\center
\scalebox{0.71}{
\begin{tabular}{|c|c|c|c|}
\hline
    & \textbf{Precision} & \textbf{Recall} & \textbf{F1}   \\ \hline
Entailment Modeling    & 0.33      & 0.71   & \textbf{0.45} \\ \hline
%Entailment Modeling w/o perturbing &0.34 &0.43 & \textbf{0.46} \\ \hline
Context Modeling      & 0.31      & 0.56   & 0.38 \\ \hline
%Cntext Modeling w/o perturbing &0.35 &0.50 &0.39 \\ \hline
GMM & \textbf{0.37}      & 0.34   & 0.35 \\ \hline

\end{tabular}}
\caption{Sentence Selection Results}
\label{table:sentence_selection_result}
\end{table}








			\begin{comment}
			\begin{table}[h!]\scalebox{0.85}{
			\begin{tabular}{|l|l|l|l|}
			\hline
			ALL SET - MH     & Precision & Recall & F1   \\ \hline
			Entailment    & 0.33      & 0.71   & 0.45 \\ \hline
			Context       & 0.31      & 0.56   & 0.38 \\ \hline
			GiveMeExample & 0.37      & 0.34   & 0.35 \\ \hline
			\end{tabular}}
			\caption{Model Sentence Selection Result vs Expert Choice}
			\label{table:sentence_selection_result}

			\end{table}

			\begin{table}[h!]\scalebox{0.85}{
			\begin{tabular}{|l|l|l|l|}
			\hline
			MOST COMMON -MH   & Precision & Recall & F1   \\ \hline
			Entailment    & 0.31      & 0.29   & 0.30 \\ \hline
			Context       & 0.34      & 0.31   & 0.32 \\ \hline
			GiveMeExample & 0.37      & 0.34   & 0.35 \\ \hline
			\end{tabular}}
			\caption{Model Sentence Selection Result vs Expert Choice}
			\label{table:sentence_selection_result-2}
			\end{table}

			\begin{table}[h!]\scalebox{0.85}{
			\begin{tabular}{|l|l|l|l|}
			\hline
			MOST COMMON-Herman & Precision & Recall & F1   \\ \hline
			Entailment         & 0.29      & 0.29   & 0.29 \\ \hline
			Context            & 0.33      & 0.33   & 0.33 \\ \hline
			GiveMeExample      & 0.28      & 0.29   & 0.29 \\ \hline
			\end{tabular}}
			\end{table}

			\begin{table}[h!]\scalebox{0.85}{
			\begin{tabular}{|l|l|l|l|}
			\hline
			All set-Herman & Precision & Recall & F1   \\ \hline
			Entailment     & 0.32      & 0.73   & 0.43 \\ \hline
			Context        & 0.32      & 0.58   & 0.40 \\ \hline
			GiveMeExample  & 0.28      & 0.29   & 0.29 \\ \hline
			\end{tabular}}
			\end{table}


			\joy{Discussion?}

			\end{comment}


==> introduction-orig.tex <==
Many English-as-a-second language learners often have trouble using
near-synonym words correctly. Near-synonyms refers to words whose meaning are
similar, but not identical to that of another term, such as \textit{establish}
and \textit{construct}. During the language learning process, an experience
common to many ESL learners is looking for example sentences to learn how two
nearly synonymous words differ. 
To help the learner's learning process, we focus on: \textbf{searching example
sentences to clarify English near synonyms}.

In previous work, researchers have developed linguistic search engines such as
Linggle~\cite{boisson2013linggle} and Netspeak\footnote{\scriptsize
www.netspeak.org} to allow users to query the word in terms of n-gram frequency
easily. However, these tools do not provide educational examples.
Some prior work also attempts to retrieve example sentences for dictionary
entries~\cite{kilgarriff2008gdex}  automatically while finding clarifying
examples for near-synonyms is not the goal. One of the few works retrieving
useful examples for near-synonyms is from Huang et
al.~\shortcite{huang2017towards}, which defines a clarification score for a
given English sentence and uses it to recommend sentences automatically.
However, most of these approaches only rely on question context and hence
providing more example sentences is not helpful. Still less their sentence
selection process depends on handcraft scoring function that may work well for
all near-synonym sets. 

While searching for a better solution, we notice that learners learn better
with useful learning materials, represented by their exam scores, while bad
materials cause confusion. 
Such behavior can be used to assess the helpfulness of example sentences.
%That is, a material can be considered good if learners achieve better performance and vice versa. 
Therefore, we proposed a \textbf{learner-like agent} which mimics human
learning behavior to enable the ability of selecting good example sentences.
Furthermore, we find effective learning originated from the capability of
inference instead of memorization.
In this task, it refers to the ability to answer questions according to the
example sentences for learning.
Therefore, we transform this research problem to an entailment problem, i.e.,
\ent{}.
Moreover, to encourage the learner-like behavior, we propose perturbing
instances for model training.
%The perturbing instances were basically negative examples but with inverse labels.
We conduct the lexical choice experiment and the behavior check experiment to
show the proposed \ent{} is superior than the commonly seen \fitb{}. In
addition, we show that perturbing instances do encourage the learner-like
behavior and hence improve the sentence assessment ability using the sentence
selection experiment. Last, the user study is conducted to study the
near-synonym learning effectiveness when deploying the proposed agent on
students.
% We further applied the learner-like agent on a sentence selection task to examine if the learner's behavior can be used to identify good material.
% Compared with the expert's choice, our model outperformed the previous work and achieved an F1 score of 0.45.
% In the user study, students learning from our learner-like agent improve the score of more than 17\%.
Our contributions are three folds:
\begin{itemize}
\item We propose a learner-like agent with perturbing instances to effectively
model learner behavior\vspace{-2mm}
\item We proposed the inference-based \ent{} instead of \fitb{} to learn the
nuance between near-synonyms.
\item We construct the first dataset of helpful example sentence assessment for
ESL learners. 
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\begin{comment}
			Thus, to solve example sentence extraction, we proposed to look at example sentences to answer questions, called \textbf{learner-like agent}, to mimic human behavior.

			% \cy{mimic human learning -> inference -> entailment problem -> not just memorizing -> perturbing instance}

			% We especially incorporate the concept of textual entailment problem with learning from example through \ent on the learner-like agent. Such a method inference the relation between the example and the question of the target word.

			% We evaluate whether our model can react to learning material quality in behavior check (Sect \ref{subsec:behave-check}). When a model can mimic human behavior, we apply it to sentence selection (Sect \ref{subsec:sentence-selection}) and compare the result with the expert's choice. Moreover, through the user study (Sect \ref{sec:learner}), we also checked whether the selected sentences are helpful to learners.

			%\cy{1. Proposed a Learner-like Agent to mimic human's behavior. 2. Collected the first confusing word clarification sentences dataset.}

			\end{comment}

